Localized quasiparticles in a fluxonium with quasi-two-dimensional amorphous kinetic inductors

Disordered superconducting materials with high kinetic inductance are an important resource to generate nonlinearity in quantum circuits and create high-impedance environments. In thin films fabricated from these materials, the combination of disorder and the low effective dimensionality leads to increased order parameter fluctuations and enhanced kinetic inductance values. Among the challenges of harnessing these compounds in coherent devices are their proximity to the superconductor-insulator phase transition, the presence of broken Cooper pairs, and the two-level systems located in the disordered structure. In this work, we fabricate tungsten silicide wires from quasi-two-dimensional films with one spatial dimension smaller than the superconducting coherence length and embed them into microwave resonators and fluxonium qubits, where the kinetic inductance provides the inductive part of the circuits. We study the dependence of loss on the frequency, disorder, and geometry of the device, and find that the loss increases with the level of disorder and is dominated by the localized quasiparticles trapped in the spatial variations of the superconducting gap.

==> sections/sketches.tex <==


Shunt in the fluxonium: high inductance is needed (expression with $R_K$, resistance quantum), can be 
JJ array \cite{10.1063/1.4832074}
or
superconducting strip made of a high-kinetic-inductance material, such as


WSi is a promising material for quantum technology applications because


WSi detectors \cite{Seleznev_2016, chiles_2020, cecil_2012}
To investigate the material properties of WSi, we fabricated resonators...
Necessity: low loss at the qubit frequency


amorphous WSi, f0 goes up first here as well \cite{compactmultimode} and here too (with SC qubit loss inconsistency!!!): \cite{Chang2013}

% activation of quasiparticles

% dominant dissipation source

% At millikelvin temperatures and single photon power, 

% at single-photon excitation / photon population

% microwave dissipation

% typical S21 response of
% examine the behavior in fluxonium circuit 


% intrinsic property of disorder within the film

% a surface distribution of TLSs

% dominant cause of loss

 with parameters of … \TK{Data for the resonances int he middle is from the Al 100 pH/sq October batch. Fits for $Q-f_0$: $\delta(f_0)=a/\sqrt{f_0}+b$. Parameters from the fit [a,b](300 pH, 100 pH Al, 100 pH Nb)=[2.13e-4,1.3e-13] [4.14e-5,7.7e-13] [9.27e-5,8.3e-13]}

\subsection{Methods}


Resonators were fabricated ...
- on what wafer
- different ground planes (Nb/Al), First Al/Nb, then WSi?
- sputter deposition/e-beam evaporation?
- film thicknesses
- strip width
- lumped and distributed
- patterning (e-beam lithography, RIE with XXX gas?)

\TL{Devices are fabricated by first depositing WSi on IPA/Acetone cleaned C-plane sapphire wafers. WSi is cosputtered, with the power applied to the two guns resulting in $\text{W}_{0.85}\text{Si}_{0.15}$. Finally, a thin (approximately 2nm thick) capping layer of silicon is deposited to prevent aging. After deposition, we pattern resist (SPR660) and deposit liftoff gold alignment marks on the wafer. The wafer is then patterned again and a short SF6 reactive ion etch is used to remove unwanted WSi.  A final round of optical lithography with LOR/SPR660 is used for the deposition of liftoff Aluminum for the ground plane and capacitance pads. In order to make contact between WSi and Al, an in situ RF clean is used. For fluxonium devices, we spin a PMGI/PMMA bilayer which we pattern with EBL and subsequently perform standard double angle aluminum junction depositions.}
Tc of WSi?
\textbf{Determination of the kinetic inductance}

Finite-element simulations in Sonnet (changing Lkin such that f0 matches the measured f0?) 

- Geometric and kinetic inductance, lumped equivalent capacitance of stripline resonators

- The characteristic impedance of the resonators

- Kinetic inductance dominates over geometric inductance. the kinetic inductance participation ratio?
(see the table from OneNote for the 300 pH film;
 see the simple ribbon Lgeo formula in the ppt for comparison)

Show the scaling of the kinetic inductance with layer thickness and strip width?

Matching the kinetic inductance values to another method? e.g. DC measurements, Ic?

Point out: in the lumped resonator, the E field is originating from/ending in the capacitor pads, which are made of Alu, not WSi
\textbf{Evaluation of the resonance curves}
\begin{enumerate}
    \item Conversion from dBm to V, deg to rad
    \item Normalizing magnitude to 1; unwrapping phase removing slope
    \item Using loopfit to fit the curves, allowing nonlinearity to extract quality factors, these are later used to calculate photon numbers. Link to package: \url{https://github.com/zobristnicholas/loopfit}
    \item Manual correction if needed (restricting fit interval [box modes close to resonance], playing with guess and tolerance)
    \item For the resonance frequency shift fixing nonlinearity to zero, this should be double checked at high powers
\end{enumerate}
Photon number calculations:
\begin{enumerate}
    \item Extract Q factors with loopfit
    \item Estimation of incoming power at the resonators: $P_{\mathrm{in}}=$VNA output power$-$discrete attenuator on the VNA output (10 or 20 dB)$-$line attenuation using quadratic polyfit on 3 points of the down going line
    \item Use $P_{\mathrm{in}}$ at eq. (\ref{eq:ph_num})
\end{enumerate}
Loopfit cites:
\cite{Swenson_nonlinear}
\cite{Geerlings}

All frequency sweeps are done with increasing frequency (makes a difference in the bifurcation regime).

We dot not use mixer calibration.

Assumed: coupling does not exhibit nonlinearity

Current of the resonators? We should check that we are in the $I\ll I_C$ limit, otherwise the bifurcated fit method is invalid.

%\rowcolors{1}{}{lightgray}
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c}
         Symbol & Variable in the code & Quantity & Reference\\
         \hline
         \hline
         $f_{\mathrm{r}, 0}$&  \texttt{pr[f0]}& low-power resonant frequency &\\
 $x_0=(f-f_{\mathrm{r}, 0})/{f_{\mathrm{r}, 0}}$& \texttt{x0} &applied detuning&Eq. (5) in L.J. Swenson et al.\\
 $x=(f-f_{\mathrm{r}})/{f_{\mathrm{r}}}$& \texttt{x}, calculated by detuning()& detuning&Eq. (2) in L.J. Swenson et al.\\
         $Q_i$&  \texttt{pr[qi]}& internal quality factor &\\
         $Q_c$&  \texttt{pr[qc]}& coupling quality factor &\\
 $Q_r = Q_i Q_c/(Q_i+Q_c)$& \texttt{q0}& total quality factor&\\
         $\sqrt{a}$&  \texttt{pd[a\_{sqrt}]}&  square root of the inductive nonlinearity&Eq. (12) in L.J. Swenson et al.\\
 $x_a$& \texttt{pr[xa]}&  resonance asymmetry &\\
 & & &\\
    \end{tabular}
    \caption{Correspondence between the notation in the formulas and variables implemented in the fitting code.}
    \label{tab:notation}
\end{table*}
If $a=0$, the applied detuning is the same as the detuning, irrespectively to the power.

In L.J. Swenson et al. the quantities are defined using angular frequencies.

Baseline:
$$
(\texttt{gain0}+ \texttt{gain1} \cdot \texttt{xm} + \texttt{gain2} \cdot \texttt{xm}^2) e^{i( \texttt{phase0} + \texttt{phase1} * \texttt{xm})}
$$

$$
({g_0}+ g_1 \cdot x_m +g_2 \cdot x_m^2) \cdot e^{i(p_0 + p_1\cdot x_m)}
$$

$$
x_m = (f-f_m)/f_m
$$
$f_m$: arbitrary parameter (median frequency of the frequency sweep by default)

Resonance function:
$$
S_{21} = 
1-\frac{{Q_r}/{Q_c}-2 i Q_0 x_a}{1+2 i Q_0 x}
=
\frac{Q_c + 2i Q_i Q_c (x+x_a)}
{Q_i + Q_c + 2i Q_i Q_c x},
$$
where the first form is  from reference  \cite{Geerlings} , the second one is the formula implemented in the code (\texttt{resonance()} function), and can be easily derived by substituting $Q_r$ and applying identical transformations.

Eq. (13) in L.J. Swenson et al. (in the detuning() function):
$$
4y^3 -4 y_0 y^2 + y - y_0 - a = 0
$$

\textbf{Determination of the photon number in the resonator}

After extracting the resonator parameters by fitting the resonance curve, we determine the photon number in the resonator \cite{Bruno_photon, cecile_nbn}:
\begin{equation}
    \label{eq:ph_num}
    \left\langle n_{\mathrm{ph}}\right\rangle=\frac{2}{\hbar \omega_0^2} \frac{Q_l^2}{Q_{\mathrm{c}}} P_{\mathrm{in}},
\end{equation}
where $P_{\mathrm{in}}$ is the microwave power incident on the resonator. We calculate $P_{\mathrm{in}}$ by correcting the VNA output power with the frequency-dependent attenuation of the input line measured at room temperature. Since the attenuation of the line decreases at low temperatures, $\left\langle n_{\mathrm{ph}}\right\rangle$ calculated with this approximation is an upper estimate. \todo{(At this point $Q_i$, $Q_c$ should be already defined.)}

\begin{equation}
1/T_1^\mathrm{ind} = 4\pi \cdot \frac{E_L/h}{Q_L} \left|\langle0|\varphi|1\rangle\right|^2 \coth{\left(\frac{h f}{2 k_BT}\right)}
\end{equation}

\subsection{Inductive loss for supplement}

Here, for completeness, we summarize the losses in a junction array arising from quasiparticles tunneling across the individual junctions based on the results published in Ref.~\cite{catelani_relaxation_2011,catelani_quasiparticle_2011}. When considering only a single junction, the coupling between the quasiparticles in the leads and the qubit degree of freedom reads
\begin{equation}
\hat{H}_T = i t\sum_{i,j,\sigma} \sin{\frac{\hat{\varphi}}{2}}\hat{\alpha}^{L\dagger}_{i,\sigma}\hat{\alpha}^{R}_{j,\sigma} + \mathrm{h.c.},
\end{equation}
where $t$ is the electron tunneling amplitude, $\hat\varphi$ is the phase difference of the superconducting order parameter across the junction and $\hat{\alpha}^{L/R}_{i,\sigma}$ describes the annihilation operator for a quasiparticle in the left/right leads in energy level $n$ and with spin $\sigma$. Based on Fermi's golden rule, the coupling Hamiltonian leads to an energy relaxation rate of 
\begin{equation}
    \Gamma_{i\rightarrow f} = \left|\left\langle i \left| \sin{\frac{\hat{\varphi}}{2}} \right| f \right\rangle\right | ^2\cdot S_\mathrm{qp}(\omega),
\end{equation}
where $|i\rangle$ and $|f\rangle$ are the initial and final states. Here, the normalized quasiparticle current spectral density is 
\begin{equation}
    S_\mathrm{qp}(\omega) = x_\mathrm{qp}\frac{8E_J}{\pi\hbar}\sqrt\frac{2\Delta}{\hbar\omega},
\end{equation}
where $x_\mathrm{qp}$ is the quasiparticle density normalized by the density of Cooper pairs, and we assumed that $k_B T \ll \hbar\omega \ll \Delta$.

In a Josephson junction array containing $N$ junctions, such quasiparticle tunneling events can happen across any of the individual junctions. Following Ref.~\cite{catelani_relaxation_2011}, we assume that each junction in the array has the same Josephson energy, $E_{J,S}$, which is much larger than the Josephson energy of the black-sheep junction, $E_J$. In this case, the array acts as a linear inductor with inductive energy of $E_L=E_{J,S} / N$.  If the plasma frequency corresponding to the junctions in the array is at a much higher energy than the qubit frequency, the phase drop across each junction can be linearized and the transition rate due to quasiparticle loss in the array is
\begin{equation}
    \Gamma_{i\rightarrow f} = \left|\left\langle i \left| \hat{\varphi} \right| f \right\rangle\right | ^2\cdot S_\mathrm{qp}^L(\omega),
\end{equation}
where 
\begin{equation}
    S_\mathrm{qp}^L(\omega)  = x_\mathrm{qp}\frac{2E_L}{\pi\hbar}\sqrt\frac{2\Delta}{\hbar\omega}.
\end{equation}

We can compare this result with a phenomenological model of inductive losses [Masluk thesis, Smith]. In this picture, we model a lossy inductor as an element that has an inductive part with inductance $L$ and a resistive component with resistance $R(\omega)$ in series with a total impedance of $Z_\mathrm{ind} (\omega) = i\omega L + R(\omega)$. The quality factor of the inductor is the ratio of the real and imaginary components
\begin{equation}
    Q_\mathrm{ind}(\omega) = \frac{\omega L}{R(\omega)}.
\end{equation}

If a lossy inductor is embedded in the fluxonium, the phase across the junction couples to the current across the inductor
\begin{equation}
    \hat{H}_C = \frac{\phi_0}{2\pi} \hat\varphi \hat{I},
\end{equation}
which leads to a relaxation rate of
\begin{equation}
    \Gamma_{i\rightarrow f} = \left|\left\langle i \left| \hat{\varphi} \right| f \right\rangle\right | ^2\cdot \frac{1}{4e^2}S_\mathrm{II}(\omega)
\end{equation}
where the quantum current noise spectral density in the $k_B T \ll \hbar\omega$ limit
\begin{equation}
    S_\mathrm{II}(\omega) = 2 \hbar\omega \mathrm{Re}\left[Y(\omega)\right].
\end{equation}
After expressing the admittance of the lossy inductor, $\left[Y(\omega)\right]\approx 1/ \omega L Q_\mathrm{ind}(\omega)$, we obtain the relaxation rate 
\begin{equation}
     \Gamma_{i\rightarrow f} = \left|\left\langle i \left| \hat{\varphi} \right| f \right\rangle\right | ^2\cdot \frac{2E_L}{\hbar Q_\mathrm{ind}(\omega)}
\end{equation}
By comparing Eqs., we find that quasiparticle tunneling across the junction array leads to an inductive loss with quality factor of
\begin{equation}
    \frac{1}{Q_\mathrm{ind}(\omega)} = \frac{1}{\pi} \sqrt{\frac{2\Delta}{\hbar\omega}} \cdot x_\mathrm{qp}
\end{equation}


